Lens mass estimate in the Galactic disk extreme parallax microlensing event Gaia19dke

We present the results of our analysis of Gaia19dke, an extraordinary microlensing event in the Cygnus constellation that was first spotted by the {\gaia} satellite. This event featured a strong microlensing parallax effect, which resulted in multiple peaks in the light curve. We conducted extensive photometric, spectroscopic, and high-resolution imaging follow-up observations to determine the mass and the nature of the invisible lensing object. Using the Milky Way priors on density and velocity of lenses, we found that the dark lens is likely to be located at a distance of $D_L =(3.05^{+4.10}_{-2.42})$kpc, and has a mass of $M_L =(0.51^{+3.07}_{-0.40}) M_\odot$. Based on its low luminosity and mass, we propose that the lens in Gaia19dke event is an isolated white dwarf.

==> tables.tex <==
\begin{table*}
        \centering
         \begin{tabular}{c c c c}
            \hline
            \noalign{\smallskip}
            Parameter & Value \\
            \noalign{\smallskip}
            \hline
            \hline
            \noalign{\smallskip}
            $t_\mathrm{0, par}$ [Reduced JD] & $9070.00$ \\
            $t_0$ [Reduced JD] & $9063.82^{+0.84}_{-0.84}$\\
            \noalign{\smallskip}
            $t_\mathrm{E}$ [days] &  $156.20^{+7.39}_{-6.89}$ \\
            \noalign{\smallskip}
            $u_0$ & $-0.6449^{+0.0539}_{-0.0578}$  \\
            \noalign{\smallskip}
            $\pi_\mathrm{EN}$ & $-0.0991^{+0.0041}_{-0.0042}$  \\
            \noalign{\smallskip}
            $\pi_\mathrm{EE}$ & $-0.1995^{+0.0083}_{-0.0084}$ \\
            \noalign{\smallskip}
            $mag_{0}$[Gaia] [mag] & $15.5059^{+0.0015}_{-0.0015}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}, G}$ & $1.0960^{+0.1696}_{-0.1434}$  \\
            \noalign{\smallskip}
            $\chi^2$ &393.43 \\
            $\frac{\chi^2}{dof}$ & 3.20\\
            \noalign{\smallskip}
            \hline
        \end{tabular}
        \caption{Parameter values of best fitting solutions for Gaia19dke using only Gaia photometric data.}
        \label{}
\end{table*}
\begin{table*}
        \centering
         \begin{tabular}{c c c c}
            \hline
            \noalign{\smallskip}
            Parameter & Value \\
            \noalign{\smallskip}
            \hline
            \hline
            \noalign{\smallskip}
            $t_\mathrm{0, par}$ [Reduced JD] & $9070.00$ \\
            $t_0$ [Reduced JD] & $9063.51^{+0.29}_{-0.29}$\\
            \noalign{\smallskip}
            $t_\mathrm{E}$ [days] &  $161.69^{+3.41}_{-2.96}$ \\
            \noalign{\smallskip}
            $u_0$ & $-0.6011^{+0.0189}_{-0.0170}$  \\
            \noalign{\smallskip}
            $\pi_\mathrm{EN}$ & $-0.0976^{+0.0019}_{-0.0017}$  \\
            \noalign{\smallskip}
            $\pi_\mathrm{EE}$ & $-0.1947^{+0.0040}_{-0.0036}$ \\
            \noalign{\smallskip}
            $mag_{0}$[Gaia] [mag] & $15.5078^{+0.0012}_{-0.0012}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[Gaia] & $0.9800^{+0.0464}_{-0.0498}$  \\
            \noalign{\smallskip}
            $mag_{0}$[Moletai i] [mag] & $14.9180^{+0.0042}_{-0.0042}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[Moletai i] & $0.8797^{+0.0414}_{-0.0442}$  \\
            \noalign{\smallskip}
            $mag_{0}$[Moletai r] [mag] & $15.5110^{+0.0046}_{-0.0045}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[Moletai r] & $0.9105^{+0.0427}_{-0.0459}$  \\
            \noalign{\smallskip}
            $mag_{0}$[Moletai V] [mag] & $15.9893^{+0.0051}_{-0.0051}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[Moletai V] & $0.9315^{+0.0443}_{-0.0468}$  \\
            \noalign{\smallskip}
            $mag_{0}$[LCOGT1m g] [mag] & $16.5082^{+0.0044}_{-0.0045}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[LCOGT1m g] & $0.9025^{+0.0410}_{-0.0438}$  \\
            \noalign{\smallskip}
            $mag_{0}$[LCOGT1m i] [mag] & $15.0148^{+0.0040}_{-0.0039}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[LCOGT1m i] & $0.9487^{+0.0421}_{-0.0457}$  \\
            \noalign{\smallskip}
            $mag_{0}$[LCOGT1m r] [mag] & $15.4973^{+0.0063}_{-0.0061}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[LCOGT1m r] & $0.9655^{+0.0448}_{-0.0471}$  \\
            \noalign{\smallskip}
            $mag_{0}$[ZTF g] [mag] & $16.5396^{+0.0018}_{-0.0018}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[ZTF g] & $0.9663^{+0.0446}_{-0.0479}$  \\
            \noalign{\smallskip}
            $mag_{0}$[ZTF i] [mag] & $14.9162^{+0.0450}_{-0.0452}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[ZTF i] & $1.0261^{+0.2062}_{-0.1950}$  \\
            \noalign{\smallskip}
            $mag_{0}$[ZTF r] [mag] & $15.3982^{+0.0014}_{-0.0013}$\\
            \noalign{\smallskip}
            $f_{\mathrm{s}}$[ZTF r] & $0.9696^{+0.0443}_{-0.0478}$  \\
            \noalign{\smallskip}
            $\chi^2$ &5418.35 \\
            $\frac{\chi^2}{dof}$ & 2.80\\
            \noalign{\smallskip}
            \hline
        \end{tabular}
        \caption{Parameter values of best fitting solutions for Gaia19dke using Gaia and follow-up photometric data.}
        \label{tab:valSolutionsGaiaFol}
\end{table*}

\begin{table}
        \centering
         \begin{tabular}{c c c}
            \hline
            \noalign{\smallskip}
            Parameter & Value\\
            \noalign{\smallskip}
            \hline
            \hline
             \noalign{\smallskip}
             \multicolumn{2}{c}{Mass function $\propto M^{-1.75}$} \\
             \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $M_\mathrm{L} \, [M_\odot]$ & $1.91^{+1.93}_{-0.97}$ \\
            \noalign{\smallskip}
            $D_\mathrm{L}$~[kpc] & $0.92^{+0.61}_{-0.41}$\\
            \hline
        \end{tabular}
        \caption{Lens mass $M_L$ and distance $D_L$ for best fitting model for Gaia19dke assuming distance do the source $3.0~\mathrm{kpc} < D_S < 5.6~\mathrm{kpc}$ and \newline mass function $\propto M^{-1.75}$.}
\end{table}

\begin{table}
        \centering
         \begin{tabular}{c c c}
            \hline
            \noalign{\smallskip}
            Parameter & Value\\
            \noalign{\smallskip}
            \hline
            \hline
             \noalign{\smallskip}
             \multicolumn{2}{c}{Mass function $\propto M^{-1.00}$} \\
             \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $M_\mathrm{L} \, [M_\odot]$ & $2.71^{+2.14}_{-1.38}$ \\
            \noalign{\smallskip}
            $D_\mathrm{L}$~[kpc] & $1.43^{+0.70}_{-0.58}$\\
            \hline
        \end{tabular}
        \caption{Lens mass $M_L$ and distance $D_L$ for best fitting model for Gaia19dke assuming distance do the source $3.0~\mathrm{kpc} < D_S < 5.6~\mathrm{kpc}$ and \newline mass function $\propto M^{-1.00}$.}
\end{table}

\begin{table}
        \centering
         \begin{tabular}{c c c}
            \hline
            \noalign{\smallskip}
            Parameter & Value\\
            \noalign{\smallskip}
            \hline
            \hline
             \noalign{\smallskip}
             \multicolumn{2}{c}{Mass function $\propto M^{-3.00}$} \\
             \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $M_\mathrm{L} \, [M_\odot]$ & $1.04^{+1.07}_{-0.51}$ \\
            \noalign{\smallskip}
            $D_\mathrm{L}$~[kpc] & $1.43^{+0.70}_{-0.58}$\\
            \hline
        \end{tabular}
        \caption{Lens mass $M_L$ and distance $D_L$ for best fitting model for Gaia19dke assuming distance do the source $3.0~\mathrm{kpc} < D_S < 5.6~\mathrm{kpc}$ and \newline mass function $\propto M^{-3.00}$.}
\end{table}
